TabPert: An Effective Platform for Tabular Perturbation

To truly grasp reasoning ability, a Natural Language Inference model should be evaluated on counterfactual data. TabPert facilitates this by assisting in the generation of such counterfactual data for assessing model tabular reasoning issues. TabPert allows a user to update a table, change its associated hypotheses, change their labels, and highlight rows that are important for hypothesis classification. TabPert also captures information about the techniques used to automatically produce the table, as well as the strategies employed to generate the challenging hypotheses. These counterfactual tables and hypotheses, as well as the metadata, can then be used to explore an existing model's shortcomings methodically and quantitatively.

==> 7_bits_figure.tex <==
\begin{table*}
%\caption{Strategy: Change table to flip label}
\centering
\begin{tabular}{p{1.5cm}|p{1.5cm}| p{1.5cm}|p{1.5cm}}
\hline \hline
 Bit Number & Location & Same Location: Bit is 0 & Other Location: Bit is 1\\
\hline
1 & Dataset & Training Set & Test $\alpha_1$ \\
2 & Category & Same Category & Different Category\\
3 & Table & Same Table & Different Table \\
4 & Key & Same Key & Different Key \\
\hline
\end{tabular}
\label{table:fourbits}
\caption{First Four Bits of Table Value Meta-Data}
\end{table*}





% \overfullrule=0mm
% \begin{tikzpicture}[grow=down, level distance = 1.5cm,
% level 1/.style = {sibling distance = 8cm},
% level 2/.style = {sibling distance = 4cm},
% level 3/.style = {sibling distance = 3cm},
% level 4/.style = {sibling distance = 2cm},]
% \node[text width=4cm,align=center] {InfoTabS Dataset}
%     child { 
%         node[text width=8cm,align=center] {Training Set}
%             child {
%                 node[text width=4cm,align=center] {Different Category }
%                     child {
%                         node[text width=1.3cm,align=center] {Different\\ Table}
%                             child {
%                                 node[text width=1.3cm,align=center] {Different\\ Key}
%                                 node[label=below:1111,yshift=-0.4cm]{}
%                                 edge from parent
%                                     node[left, xshift=-0.1cm] {1}
%                             }
%                             child {
%                                 node[text width=1.3cm,align=center] {Same\\ Key}
%                                 node[label=below:1110,yshift=-0.4cm]{}
%                                 edge from parent
%                                     node[right, xshift=0.1cm] {0}
%                             }
%                             edge from parent
%                                 node[left, xshift=-0.1cm] {1}
%                     }
%                     edge from parent
%                         node[left, xshift=-0.3cm] {1}
%             }
%             child {
%                 node[text width=4cm,align=center] {Same Category }
%                     child {
%                         node[text width=1.3cm,align=center] {Different Table}
%                             child {
%                                 node[text width=1.3cm,align=center] {Different Key}
%                                 node[label=below:1011,yshift=-0.4cm]{}
%                                 edge from parent
%                                     node[left, xshift=-0.1cm] {1}
%                             }
%                             child {
%                                 node[text width=1.3cm,align=center] {Same Key} node[label=below:1010,yshift=-0.4cm]{}
%                                 edge from parent
%                                     node[right, xshift=0.1cm] {0}
%                             }
%                             edge from parent
%                                 node[left, xshift=-0.1cm] {1}
%                     }
%                     edge from parent
%                         node[left, xshift=0.65cm] {0}
%             }
%             edge from parent
%                 node[left, xshift=-0.5cm] {1}
%     }
%     child {
%         node[text width=6cm,align=center] {Test $\alpha_1$ Set}
%             child {
%                 node[text width=4cm,align=center] {Different Category}
%                     child {
%                         node[text width=1.3cm,align=center] {Different Table}
%                             child {
%                                 node[text width=1.3cm,align=center] {Different Key}
%                                 node[label=below:0111,yshift=-0.4cm]{}
%                                 edge from parent
%                                     node[left, xshift=-0.1cm] {1}
%                             }
%                             child {
%                                 node[text width=1.3cm,align=center,xshift=-0.4cm] {Same Key}
%                                 node[label=below:0110,yshift=-0.4cm,xshift=-0.4cm]{}
%                                 edge from parent
%                                     node[right, xshift=0.1cm] {0}
%                             }
%                             edge from parent
%                                 node[left, xshift=-0.1cm] {1}
%                     }
%                     edge from parent
%                         node[left, xshift=-0.3cm] {1}
%             }
%             child {
%                 node[text width=4cm,align=center] {Same Category }
%                     child {
%                         node[text width=1.3cm,align=center] {Different Table}
%                             child {
%                                 node[text width=1.3cm,align=center,xshift=0.3cm] {Different Key}
%                                 node[label=below:0011,yshift=-0.4cm,xshift=0.3cm]{}
%                                 edge from parent
%                                     node[left, xshift=-0.1cm] {1}
%                             }
%                             child {
%                                 node[text width=1.3cm,align=center,xshift=-0.3cm] {Same Key}
%                                 node[label=below:0010,yshift=-0.4cm,xshift=-0.3cm]{}
%                                 edge from parent
%                                     node[right, xshift=0.1cm] {0}
%                             }
%                             edge from parent
%                                 node[left, xshift=-0.1cm] {1}
%                     }
%                     child {
%                         node[text width=1.3cm,align=center] {Same Table}
%                             child {
%                                 node[text width=1.3cm,align=center] {Different Key}
%                                 node[label=below:0001,yshift=-0.4cm]{}
%                                 edge from parent
%                                     node[left, xshift=-0.1cm] {1}
%                             }
%                             child {
%                                 node[text width=1.3cm,align=center] {Same Key}
%                                 node[label=below:0000,yshift=-0.4cm]{}
%                                 edge from parent
%                                     node[right, xshift=0.1cm] {0}
%                             }
%                             edge from parent
%                                 node[right, xshift=0.1cm] {0}
%                     }
%                     edge from parent
%                         node[left, xshift=0.65cm] {0}
%             }
%             edge from parent
%                 node[right, xshift=0.5cm] {0}
%     };

% \end{tikzpicture}
